Enhancing Robustness of Machine Learning Systems via Data Transformations

We propose the use of data transformations as a defense against evasion attacks on ML classifiers. We present and investigate strategies for incorporating a variety of data transformations including dimensionality reduction via Principal Component Analysis and data `anti-whitening' to enhance the resilience of machine learning, targeting both the classification and the training phase. We empirically evaluate and demonstrate the feasibility of linear transformations of data as a defense mechanism against evasion attacks using multiple real-world datasets. Our key findings are that the defense is (i) effective against the best known evasion attacks from the literature, resulting in a two-fold increase in the resources required by a white-box adversary with knowledge of the defense for a successful attack, (ii) applicable across a range of ML classifiers, including Support Vector Machines and Deep Neural Networks, and (iii) generalizable to multiple application domains, including image classification and human activity classification.

==> Acknowledgements.tex <==
We would like to thank Chawin Sitawarin for help with experiments and useful discussions. Arjun Nitin Bhagoji is supported by NSF and DARPA. Daniel Cullina is supported by DARPA.

==> datafigures/plots/fg_cnn_9_papernot_strat_rev_pca_.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,1111){\makebox(0,0)[r]{\strut{} 20}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,1518){\makebox(0,0)[r]{\strut{} 40}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,1925){\makebox(0,0)[r]{\strut{} 60}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,2332){\makebox(0,0)[r]{\strut{} 80}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,2739){\makebox(0,0)[r]{\strut{} 100}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1514,484){\makebox(0,0){\strut{} 1}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2170,484){\makebox(0,0){\strut{} 2}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2825,484){\makebox(0,0){\strut{} 3}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3481,484){\makebox(0,0){\strut{} 4}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4137,484){\makebox(0,0){\strut{} 5}}%
      \csname LTb\endcsname%
      \put(220,1721){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize{Adversarial success (\%)}}}}%
      \put(2497,154){\makebox(0,0){\strut{}$\eta = \|\bfx- \xad\|_\infty$}}%
      \put(2497,3069){\makebox(0,0){\strut{}\small{White box FG attack on CNN on MNIST with pca}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3150,2197){\makebox(0,0)[r]{\strut{}\small{None}}}%
      \csname LTb\endcsname%
      \put(3150,1977){\makebox(0,0)[r]{\strut{}\small{331}}}%
      \csname LTb\endcsname%
      \put(3150,1757){\makebox(0,0)[r]{\strut{}\small{100}}}%
      \csname LTb\endcsname%
      \put(3150,1537){\makebox(0,0)[r]{\strut{}\small{80}}}%
      \csname LTb\endcsname%
      \put(3150,1317){\makebox(0,0)[r]{\strut{}\small{60}}}%
      \csname LTb\endcsname%
      \put(3150,1097){\makebox(0,0)[r]{\strut{}\small{40}}}%
      \csname LTb\endcsname%
      \put(3150,877){\makebox(0,0)[r]{\strut{}\small{20}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{datafigures/plots/fg_cnn_9_papernot_strat_rev_pca}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> datafigures/plots/fg_mnist_nn_FC_2_100_pca_retrain_.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,1111){\makebox(0,0)[r]{\strut{} 20}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,1518){\makebox(0,0)[r]{\strut{} 40}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,1925){\makebox(0,0)[r]{\strut{} 60}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,2332){\makebox(0,0)[r]{\strut{} 80}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(726,2739){\makebox(0,0)[r]{\strut{} 100}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1514,484){\makebox(0,0){\strut{} 1}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2170,484){\makebox(0,0){\strut{} 2}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2825,484){\makebox(0,0){\strut{} 3}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3481,484){\makebox(0,0){\strut{} 4}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4137,484){\makebox(0,0){\strut{} 5}}%
      \csname LTb\endcsname%
      \put(220,1721){\rotatebox{-270}{\makebox(0,0){\strut{}\small{Adversarial success (\%)}}}}%
      \put(2497,154){\makebox(0,0){\strut{}$\epsilon = \|\bfx- \xad\|_2$}}%
      \put(2497,3069){\makebox(0,0){\strut{}\small{Classifier mismatch FG attack on NN on MNIST with pca}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1650,2566){\makebox(0,0)[r]{\strut{}\small{None}}}%
      \csname LTb\endcsname%
      \put(1650,2346){\makebox(0,0)[r]{\strut{}\small{331}}}%
      \csname LTb\endcsname%
      \put(1650,2126){\makebox(0,0)[r]{\strut{}\small{100}}}%
      \csname LTb\endcsname%
      \put(1650,1906){\makebox(0,0)[r]{\strut{}\small{80}}}%
      \csname LTb\endcsname%
      \put(1650,1686){\makebox(0,0)[r]{\strut{}\small{60}}}%
      \csname LTb\endcsname%
      \put(1650,1466){\makebox(0,0)[r]{\strut{}\small{40}}}%
      \csname LTb\endcsname%
      \put(1650,1246){\makebox(0,0)[r]{\strut{}\small{20}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{datafigures/plots/fg_mnist_nn_FC_2_100_pca_retrain}}%
    \gplfronttext
  \end{picture}%
\endgroup

